Video Instance Matting

Conventional video matting outputs one alpha matte for all instances appearing in a video frame so that individual instances are not distinguished. While video instance segmentation provides time-consistent instance masks, results are unsatisfactory for matting applications, especially due to applied binarization. To remedy this deficiency, we propose Video Instance Matting~(VIM), that is, estimating alpha mattes of each instance at each frame of a video sequence. To tackle this challenging problem, we present MSG-VIM, a Mask Sequence Guided Video Instance Matting neural network, as a novel baseline model for VIM. MSG-VIM leverages a mixture of mask augmentations to make predictions robust to inaccurate and inconsistent mask guidance. It incorporates temporal mask and temporal feature guidance to improve the temporal consistency of alpha matte predictions. Furthermore, we build a new benchmark for VIM, called VIM50, which comprises 50 video clips with multiple human instances as foreground objects. To evaluate performances on the VIM task, we introduce a suitable metric called Video Instance-aware Matting Quality~(VIMQ). Our proposed model MSG-VIM sets a strong baseline on the VIM50 benchmark and outperforms existing methods by a large margin. The project is open-sourced at https://github.com/SHI-Labs/VIM.

==> tables/ablation_mask.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{c|cccc}
Method &  RQ & TQ & MQ & VMQ \\ \hline
MTRCNN~\cite{yang2019video}  &37.43 &78.00 &15.49 &4.52  \\
MTRCNN + MGVIM  &- &- &- &- \\ \hline
SeqFormer~\cite{wu2021seqformer}  &79.83 &98.01 &36.01 &28.18 \\
SeqFormer + MGVIM &- &- &- &- \\ \hline
\end{tabular}
\caption{Ablation of Mask Guidance. We used mask guidance from outputs of MaskTrackRCNN~\cite{yang2019video} and SeqFormer~\cite{wu2021seqformer}. All models are tested on the VIM100 synthetic set.} 
\label{ablation_mask}
\end{table}

==> tables/ablation_metric.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{ccccccc}
Error & IoU & $\omega$ & RQ & TQ & MQ & VMQ \\ \hline
 MSE &0.5 &50   &72.72 &93.17 &56.52 &38.29 \\
 MSE &0.7 &50    &65.92 &86.95 &57.92 &33.20 \\
 MSE &0.5 &20    &72.72 &93.17 &70.03 &47.44 \\
 MAD &0.5 &50    &72.72 &93.17 &40.49 &27.43 \\
 dtSSD &0.5 &50   &72.72 &93.17 &5.03 &3.41 \\
 dtSSD &0.5 &10   &72.72 &93.17 &28.51 &19.32 \\
\hline
\end{tabular}
\caption{Ablations of VIMQ metrics. All of them are evaluated with the MSG-VIM model on the VIM50 benchmark.} 
\label{ablation_metric}
\end{table}

==> tables/rvm_lr_testset.tex <==
\begin{table}[tb]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|cccc}
Model &MAD &  MSE &  Grad &  Conn \\ \hline %\midrule[1.5pt]  %dtSSD\\ \hline %\midrule[1.5pt]
\multicolumn{1}{l}{\textit{LR: $512 \times 288$}} \\ \hline
DeepLabV3~\cite{chen2017rethinking} &14.47 &9.67 &8.55 &1.69 \\ % &5.18\\
FBA~\cite{forte2020f} &8.36 &3.37 &2.09 &0.75 \\ %&2.09\\
BGMv2~\cite{lin2021real} &25.19 &19.63 &2.28 &3.26 \\ %&2.74\\
MODNet~\cite{sun2021modnet} &9.41 &4.30 &1.89 &0.81 \\ %&2.23\\
RVM~\cite{lin2021robust}  &6.08 &1.47 &0.88 &0.41\\ %&1.36\\
MSG-VIM  &5.97 &2.55 &1.22 &0.56 \\ \hline %&2.47 \\ \hline 
\multicolumn{1}{l}{\textit{HD: $1920 \times 1080$}} \\ \hline
MODNet~\cite{sun2021modnet} &11.13 &5.54 &15.30 &- \\ %&3.08 \\
RVM~\cite{lin2021robust}  &6.57 &1.93 &10.55 &- \\ %&1.90 \\
MSG-VIM  &\textbf{6.47} &\textbf{1.73} &\textbf{10.40} &- %&6.59 \\ %&2.41 \\
\end{tabular}}
\caption{Performance of state-of-the-art methods  on the video matting benchmark of RVM~\cite{lin2021robust}. We evaluate MSG-VIM under input of $512 \times 288$ and $1920 \times 1080$. All metrics are the lower, the better.}
\label{rvm_lr_testet}
\end{table}
